Chemical Abundances in the Ultra-Faint Dwarf Galaxies Grus I and Triangulum II: Neutron-Capture Elements as a Defining Feature of the Faintest Dwarfs

We present high-resolution of spectroscopy of four stars in two candidate ultra-faint dwarf galaxies (UFDs) Grus I (Gru I) and Triangulum II (Tri II). Neither object currently has a clearly determined velocity dispersion, placing them in an ambiguous region of parameter space between dwarf galaxies and globular clusters. No significant metallicity difference is found for the two Gru I stars, but both stars are deficient in neutron-capture elements. We verify previous results that Tri II displays significant spreads in metallicity and [$\alpha$/Fe]. Neutron-capture elements are not detected in our Tri II data, but we place upper limits at the lower envelope of Galactic halo stars, consistent with previous very low detections. Stars with similarly low neutron-capture element abundances are common in UFDs, but rare in other environments. This signature of low neutron-capture element abundances traces chemical enrichment in the least massive star-forming dark matter halos, and further shows that the dominant sources of neutron-capture elements in metal-poor stars are rare. In contrast, all known globular clusters have similar ratios of neutron-capture elements to those of halo stars, suggesting that globular clusters form as part of relatively massive galaxies rather than in their own dark matter halos. The low neutron-capture element abundances may be the strongest evidence that Gru I and Tri II are (or once were) galaxies rather than globular clusters, and we expect future observations of these systems to robustly find non-zero velocity dispersions or signs of tidal disruption. However, the nucleosynthetic origin of this low neutron-capture element floor remains unknown.

==> ew_final.tex <==
\begin{deluxetable*}{llrrrrrrrrrrrrrrrrrr}
\tablecolumns{20}
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tabletypesize{\tiny}
\tablecaption{\label{tbl:eqw}}
\tablehead{\colhead{El.} & \colhead{$\lambda$} & \colhead{$\chi$} & \colhead{$\log gf$} & \colhead{EW} & \colhead{$\sigma(EW)$} & \colhead{$\log \epsilon$} & \colhead{$\sigma(\log\epsilon)$} & \colhead{EW} & \colhead{$\sigma(EW)$} & \colhead{$\log \epsilon$} & \colhead{$\sigma(\log\epsilon)$} & \colhead{EW} & \colhead{$\sigma(EW)$} & \colhead{$\log \epsilon$} & \colhead{$\sigma(\log\epsilon)$} & \colhead{EW} & \colhead{$\sigma(EW)$} & \colhead{$\log \epsilon$} & \colhead{$\sigma(\log\epsilon)$}\\
\colhead{} & \colhead{(\AA)} & \colhead{(eV)} & \colhead{(dex)} & \multicolumn{4}{c}{GruI-032} & \multicolumn{4}{c}{GruI-038} & \multicolumn{4}{c}{TriII-40} & \multicolumn{4}{c}{TriII-46}}
\startdata
CH    &  4313.00 &\nodata&  \nodata &     syn & \nodata &    5.45 &    0.20 &     syn & \nodata &    5.62 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
CH    &  4323.00 &\nodata&  \nodata &     syn & \nodata &    5.25 &    0.30 &     syn & \nodata &    5.58 &    0.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Na I  &  5889.95 &  0.00 & $  0.11$ &   210.7 &    29.2 &    3.59 &    0.37 &   174.9 &    24.5 &    3.44 &    0.37 &   104.9 &    16.7 &    2.49 &    0.25 &   128.3 &    42.8 &    3.41 &    0.68 \\
Na I  &  5895.92 &  0.00 & $ -0.19$ &   175.4 &    25.5 &    3.43 &    0.36 &   160.5 &    23.8 &    3.52 &    0.37 &    83.9 &    14.6 &    2.51 &    0.20 &   145.9 &    69.6 &    3.97 &    1.08 \\
Na I  &  8183.26 &  2.10 & $  0.23$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn & \nodata &$  <5.61$& \nodata \\
Na I  &  8194.82 &  2.10 & $  0.49$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn & \nodata &$  <5.15$& \nodata \\
Mg I  &  4571.10 &  0.00 & $ -5.69$ &   136.9 &    21.7 &    5.67 &    0.33 &   112.5 &    18.1 &    5.70 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mg I  &  4702.99 &  4.33 & $ -0.38$ &   105.3 &    18.6 &    5.39 &    0.28 &    88.7 &    16.9 &    5.25 &    0.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mg I  &  5172.68 &  2.71 & $ -0.45$ &   275.4 &    45.2 &    5.45 &    0.36 &   240.2 &    45.7 &    5.32 &    0.42 &   179.9 &    28.6 &    4.82 &    0.41 &   184.6 &    55.6 &    5.14 &    0.63 \\
Mg I  &  5183.60 &  2.72 & $ -0.24$ &   310.6 &    48.0 &    5.46 &    0.30 &   280.0 &    47.3 &    5.37 &    0.31 &   208.7 &    33.8 &    4.96 &    0.40 &   206.1 &    59.6 &    5.11 &    0.56 \\
Mg I  &  5528.40 &  4.34 & $ -0.50$ &    99.4 &    17.4 &    5.36 &    0.24 &    78.5 &    15.7 &    5.21 &    0.21 &    60.6 &    10.3 &    5.02 &    0.14 & \nodata & \nodata & \nodata & \nodata \\
Al I  &  3961.52 &  0.01 & $ -0.34$ &   163.2 &    65.1 &    2.97 &    1.18 &   154.6 &    78.2 &    3.08 &    1.42 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Si I  &  4102.94 &  1.91 & $ -3.14$ &   116.8 &    35.6 &    5.38 &    0.66 &   112.3 &    30.3 &    5.56 &    0.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
K I   &  7664.90 &  0.00 & $  0.14$ &   110.3 &    27.3 &    3.12 &    0.35 &   107.3 &    23.5 &    3.32 &    0.34 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
K I   &  7698.96 &  0.00 & $ -0.17$ &    81.3 &    11.4 &    3.08 &    0.14 &    77.8 &    11.3 &    3.23 &    0.15 &     syn & \nodata &    2.89 &    0.30 &     syn & \nodata &$  <3.79$& \nodata \\
Ca I  &  4425.44 &  1.88 & $ -0.36$ &    79.2 &    19.5 &    3.99 &    0.31 &    47.4 &    15.9 &    3.66 &    0.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4435.69 &  1.89 & $ -0.52$ &    49.6 &    15.2 &    3.73 &    0.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4454.78 &  1.90 & $  0.26$ &   108.4 &    22.7 &    3.87 &    0.41 &    78.1 &    17.9 &    3.51 &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  4455.89 &  1.90 & $ -0.53$ & \nodata & \nodata & \nodata & \nodata &    59.2 &    15.7 &    4.02 &    0.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  5265.56 &  2.52 & $ -0.26$ &    68.2 &    22.1 &    4.44 &    0.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  5588.76 &  2.52 & $  0.21$ &    72.4 &    14.0 &    4.01 &    0.19 & \nodata & \nodata & \nodata & \nodata &    42.5 &    12.3 &    3.77 &    0.21 & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  5594.47 &  2.52 & $  0.10$ &    54.0 &    12.8 &    3.87 &    0.19 &    43.9 &    11.3 &    3.84 &    0.19 &    31.6 &     8.4 &    3.69 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  5598.49 &  2.52 & $ -0.09$ &    51.4 &    12.5 &    4.02 &    0.19 & \nodata & \nodata & \nodata & \nodata &    42.6 &     9.7 &    4.07 &    0.16 & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  5857.45 &  2.93 & $  0.23$ & \nodata & \nodata & \nodata & \nodata &    42.6 &     9.6 &    4.17 &    0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  6102.72 &  1.88 & $ -0.79$ &    62.4 &    10.4 &    4.04 &    0.14 &    52.9 &    10.1 &    4.06 &    0.15 &    42.5 &     9.3 &    3.99 &    0.15 & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  6122.22 &  1.89 & $ -0.32$ &    83.7 &    13.1 &    3.85 &    0.18 &   100.3 &    15.6 &    4.27 &    0.23 &    55.5 &     9.0 &    3.72 &    0.13 &    55.1 &    12.9 &    4.08 &    0.21 \\
Ca I  &  6162.17 &  1.90 & $ -0.09$ &   109.8 &    15.2 &    3.98 &    0.21 &   100.0 &    14.6 &    4.04 &    0.22 &    70.8 &    10.9 &    3.71 &    0.15 &    67.6 &    18.9 &    4.06 &    0.30 \\
Ca I  &  6169.56 &  2.53 & $ -0.48$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    31.0 &     7.3 &    4.25 &    0.15 & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  6439.07 &  2.52 & $  0.47$ &    74.5 &    10.8 &    3.72 &    0.14 &    66.3 &    11.5 &    3.75 &    0.16 &    44.2 &     7.4 &    3.50 &    0.12 &    90.2 &    19.5 &    4.59 &    0.34 \\
Ca I  &  6449.81 &  2.52 & $ -0.50$ &    29.5 &     7.1 &    4.04 &    0.14 &    34.6 &     7.6 &    4.25 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ca I  &  6717.69 &  2.71 & $ -0.52$ &    26.3 &     5.7 &    4.22 &    0.13 &    20.9 &     5.6 &    4.21 &    0.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sc II &  4246.82 &  0.32 & $  0.24$ &     syn & \nodata &    0.55 &    0.50 &     syn & \nodata &    0.63 &    0.70 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sc II &  4314.08 &  0.62 & $ -0.10$ & \nodata & \nodata & \nodata & \nodata &     syn & \nodata &    0.80 &    0.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sc II &  4325.00 &  0.59 & $ -0.44$ &     syn & \nodata &    0.50 &    0.50 &     syn & \nodata &    0.57 &    0.40 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sc II &  4400.39 &  0.61 & $ -0.54$ &     syn & \nodata &    0.25 &    0.40 &     syn & \nodata &    0.96 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sc II &  4415.54 &  0.59 & $ -0.67$ &     syn & \nodata &    1.00 &    0.35 &     syn & \nodata &    0.87 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sc II &  5684.20 &  1.51 & $ -0.85$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn & \nodata &$  <0.98$& \nodata &     syn & \nodata &$  <2.65$& \nodata \\
Ti I  &  3998.64 &  0.05 & $  0.01$ & \nodata & \nodata & \nodata & \nodata &   102.7 &    34.8 &    2.57 &    0.75 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4518.02 &  0.83 & $ -0.27$ & \nodata & \nodata & \nodata & \nodata &    35.0 &    11.2 &    2.61 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4533.25 &  0.85 & $  0.53$ &    95.8 &    25.7 &    2.51 &    0.43 &    57.3 &    20.6 &    2.18 &    0.31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4534.78 &  0.84 & $  0.34$ &    75.9 &    21.3 &    2.39 &    0.32 &    48.1 &    16.2 &    2.22 &    0.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4535.57 &  0.83 & $  0.12$ &    63.0 &    18.9 &    2.42 &    0.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4555.49 &  0.85 & $ -0.43$ &    37.6 &    11.7 &    2.62 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4656.47 &  0.00 & $ -1.29$ &    64.9 &    14.0 &    2.78 &    0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4681.91 &  0.05 & $ -1.01$ &    78.5 &    14.4 &    2.73 &    0.20 &    37.4 &     9.4 &    2.42 &    0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4981.73 &  0.84 & $  0.56$ &    69.2 &    17.5 &    2.02 &    0.23 &    87.0 &    22.9 &    2.52 &    0.38 &    72.4 &    17.8 &    2.41 &    0.27 & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  4991.07 &  0.84 & $  0.44$ &   111.1 &    29.8 &    2.74 &    0.48 & \nodata & \nodata & \nodata & \nodata &    52.9 &    14.8 &    2.26 &    0.23 & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  5007.21 &  0.82 & $  0.17$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    38.5 &    11.0 &    2.29 &    0.19 & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  5173.74 &  0.00 & $ -1.06$ &    76.1 &    18.8 &    2.62 &    0.24 &    66.6 &    23.9 &    2.78 &    0.33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  5192.97 &  0.02 & $ -0.95$ &    71.2 &    19.3 &    2.48 &    0.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti I  &  5210.39 &  0.05 & $ -0.83$ &    71.4 &    16.5 &    2.39 &    0.21 &    66.2 &    16.4 &    2.60 &    0.23 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4012.40 &  0.57 & $ -1.75$ & \nodata & \nodata & \nodata & \nodata &    93.4 &    32.1 &    2.27 &    0.67 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4025.12 &  0.61 & $ -1.98$ & \nodata & \nodata & \nodata & \nodata &   108.4 &    39.5 &    2.84 &    0.85 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4161.53 &  1.08 & $ -2.16$ & \nodata & \nodata & \nodata & \nodata &    42.4 &    15.5 &    2.47 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4184.31 &  1.08 & $ -2.51$ &    55.1 &    18.1 &    2.70 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4290.22 &  1.16 & $ -0.93$ & \nodata & \nodata & \nodata & \nodata &   102.7 &    33.2 &    2.27 &    0.68 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4330.72 &  1.18 & $ -2.06$ &    97.5 &    25.0 &    3.00 &    0.46 &    59.9 &    21.1 &    2.74 &    0.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4337.91 &  1.08 & $ -0.96$ &   138.4 &    32.2 &    2.54 &    0.62 &   136.3 &    34.6 &    2.87 &    0.68 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4394.06 &  1.22 & $ -1.78$ &   102.8 &    23.0 &    2.85 &    0.43 &    77.4 &    18.2 &    2.75 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4395.03 &  1.08 & $ -0.54$ &   162.7 &    29.9 &    2.55 &    0.56 &   152.0 &    27.2 &    2.74 &    0.54 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4395.84 &  1.24 & $ -1.93$ &    60.2 &    18.3 &    2.37 &    0.27 &    57.2 &    15.2 &    2.63 &    0.23 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4399.77 &  1.24 & $ -1.19$ &   130.5 &    30.4 &    2.80 &    0.58 &   102.9 &    21.2 &    2.62 &    0.41 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4417.71 &  1.17 & $ -1.19$ &   127.4 &    26.0 &    2.64 &    0.50 &   118.5 &    26.9 &    2.83 &    0.53 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4418.33 &  1.24 & $ -1.97$ &    74.7 &    19.6 &    2.62 &    0.30 &    68.5 &    19.6 &    2.83 &    0.31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4441.73 &  1.18 & $ -2.41$ & \nodata & \nodata & \nodata & \nodata &    56.4 &    17.9 &    3.02 &    0.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4443.80 &  1.08 & $ -0.72$ & \nodata & \nodata & \nodata & \nodata &   152.6 &    28.5 &    2.91 &    0.56 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4444.55 &  1.12 & $ -2.24$ & \nodata & \nodata & \nodata & \nodata &    70.5 &    19.3 &    2.98 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4450.48 &  1.08 & $ -1.52$ &   119.0 &    21.8 &    2.68 &    0.41 &    89.8 &    18.9 &    2.51 &    0.33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4464.45 &  1.16 & $ -1.81$ &    99.7 &    24.1 &    2.73 &    0.42 &   111.5 &    26.5 &    3.28 &    0.53 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4468.52 &  1.13 & $ -0.60$ & \nodata & \nodata & \nodata & \nodata &   140.2 &    29.2 &    2.60 &    0.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4470.85 &  1.17 & $ -2.02$ &    72.2 &    18.0 &    2.53 &    0.27 &    66.8 &    21.2 &    2.77 &    0.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4501.27 &  1.12 & $ -0.77$ &   145.0 &    22.4 &    2.45 &    0.42 &   145.9 &    23.7 &    2.86 &    0.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4529.48 &  1.57 & $ -2.03$ & \nodata & \nodata & \nodata & \nodata &    45.4 &    17.2 &    2.94 &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4533.96 &  1.24 & $ -0.53$ & \nodata & \nodata & \nodata & \nodata &   145.4 &    28.1 &    2.75 &    0.56 &    98.7 &    25.5 &    1.76 &    0.48 & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4545.14 &  1.13 & $ -1.81$ & \nodata & \nodata & \nodata & \nodata &    52.5 &    14.6 &    2.30 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4563.77 &  1.22 & $ -0.96$ &   157.1 &    24.5 &    2.98 &    0.45 &   129.2 &    21.0 &    2.83 &    0.41 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4571.97 &  1.57 & $ -0.32$ & \nodata & \nodata & \nodata & \nodata &   143.0 &    22.7 &    2.89 &    0.44 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4589.91 &  1.24 & $ -1.79$ &   106.5 &    19.9 &    2.91 &    0.35 &    93.7 &    20.5 &    3.02 &    0.36 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4657.20 &  1.24 & $ -2.24$ &    68.7 &    14.2 &    2.77 &    0.20 &    47.2 &    13.6 &    2.77 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4708.66 &  1.24 & $ -2.34$ &    62.5 &    12.4 &    2.78 &    0.17 &    61.1 &    13.2 &    3.06 &    0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4779.98 &  2.05 & $ -1.37$ &    53.7 &    12.4 &    2.70 &    0.19 &    45.4 &    13.2 &    2.84 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4798.53 &  1.08 & $ -2.68$ &    76.0 &    15.5 &    3.09 &    0.22 &    46.5 &    12.3 &    2.99 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4805.09 &  2.06 & $ -1.10$ &    64.5 &    12.9 &    2.59 &    0.19 &    59.8 &    15.5 &    2.79 &    0.23 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  4865.61 &  1.12 & $ -2.81$ &    30.4 &     8.2 &    2.60 &    0.17 &    29.1 &    10.2 &    2.88 &    0.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5129.16 &  1.89 & $ -1.24$ & \nodata & \nodata & \nodata & \nodata &    60.3 &    19.1 &    2.71 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5154.07 &  1.58 & $ -1.22$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    62.7 &    22.0 &    2.99 &    0.38 \\
Ti II &  5185.90 &  1.89 & $ -1.49$ &    68.4 &    18.3 &    2.78 &    0.25 &    39.2 &    15.8 &    2.64 &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5188.69 &  1.58 & $ -1.05$ &   125.5 &    24.6 &    2.78 &    0.42 &    85.5 &    25.3 &    2.48 &    0.41 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5226.54 &  1.57 & $ -1.26$ & \nodata & \nodata & \nodata & \nodata &    66.1 &    19.9 &    2.41 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5336.79 &  1.58 & $ -1.59$ &    85.9 &    21.4 &    2.70 &    0.30 &    83.9 &    19.2 &    2.99 &    0.29 &    46.6 &    12.4 &    2.38 &    0.19 & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5381.02 &  1.57 & $ -1.92$ &    41.2 &    10.1 &    2.42 &    0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ti II &  5418.77 &  1.58 & $ -2.00$ &    30.6 &     8.3 &    2.33 &    0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4274.80 &  0.00 & $ -0.22$ & \nodata & \nodata & \nodata & \nodata &   147.6 &    38.2 &    2.77 &    0.78 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4289.72 &  0.00 & $ -0.37$ & \nodata & \nodata & \nodata & \nodata &   128.7 &    33.9 &    2.54 &    0.68 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4616.14 &  0.98 & $ -1.19$ &    48.9 &    12.0 &    2.91 &    0.18 &    31.1 &     8.2 &    2.83 &    0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4626.19 &  0.97 & $ -1.32$ &    50.6 &    11.9 &    3.05 &    0.18 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4646.15 &  1.03 & $ -0.74$ &    74.4 &    15.2 &    2.88 &    0.21 &    60.1 &    14.8 &    2.89 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  4652.16 &  1.00 & $ -1.03$ &    31.0 &    10.4 &    2.49 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5206.04 &  0.94 & $  0.02$ &   137.0 &    29.0 &    2.87 &    0.47 &   110.7 &    23.7 &    2.73 &    0.44 &    66.8 &    15.7 &    2.17 &    0.22 & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5208.42 &  0.94 & $  0.16$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   104.2 &    19.4 &    2.60 &    0.35 & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5296.69 &  0.98 & $ -1.36$ &    53.9 &    11.8 &    3.09 &    0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5298.28 &  0.98 & $ -1.14$ &    52.9 &    13.9 &    2.85 &    0.20 &    54.3 &    14.5 &    3.09 &    0.22 &    23.1 &     6.8 &    2.67 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5345.80 &  1.00 & $ -0.95$ &    66.2 &    16.1 &    2.86 &    0.22 &    45.1 &    13.7 &    2.78 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Cr I  &  5409.77 &  1.03 & $ -0.67$ &    94.4 &    18.3 &    2.97 &    0.27 &    58.4 &    15.4 &    2.73 &    0.23 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4030.75 &  0.00 & $ -0.48$ &     syn & \nodata &    2.70 &    0.50 &     syn & \nodata &    1.90 &    0.65 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4033.06 &  0.00 & $ -0.62$ &     syn & \nodata &    3.05 &    0.60 &     syn & \nodata &    1.98 &    0.70 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4034.48 &  0.00 & $ -0.81$ &     syn & \nodata &    3.05 &    0.70 &     syn & \nodata &    2.25 &    0.80 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4041.36 &  2.11 & $  0.28$ &     syn & \nodata &    2.40 &    0.50 &     syn & \nodata &    2.35 &    0.40 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4754.05 &  2.28 & $ -0.09$ &     syn & \nodata &    2.45 &    0.25 &     syn & \nodata &    2.56 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4783.43 &  2.30 & $  0.04$ &     syn & \nodata &    2.43 &    0.25 &     syn & \nodata &    2.43 &    0.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4783.43 &  2.78 & $  0.04$ &     syn & \nodata &    2.43 &    0.25 &     syn & \nodata &    2.43 &    0.25 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Mn I  &  4823.53 &  2.32 & $  0.14$ &     syn & \nodata &    2.40 &    0.20 &     syn & \nodata &    2.56 &    0.15 &     syn & \nodata &$  <2.97$& \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4139.93 &  0.99 & $ -3.63$ &    76.3 &    22.8 &    5.17 &    0.38 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4143.41 &  3.05 & $ -0.20$ &   106.5 &    30.0 &    4.90 &    0.62 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4152.17 &  0.96 & $ -3.23$ &    89.9 &    28.1 &    4.95 &    0.49 &    71.3 &    21.9 &    4.94 &    0.38 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4156.80 &  2.83 & $ -0.81$ & \nodata & \nodata & \nodata & \nodata &    74.5 &    24.5 &    4.85 &    0.46 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4175.64 &  2.85 & $ -0.83$ &    81.5 &    32.3 &    4.82 &    0.60 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4181.76 &  2.83 & $ -0.37$ &   107.4 &    23.2 &    4.80 &    0.48 &    77.9 &    24.2 &    4.47 &    0.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4187.04 &  2.45 & $ -0.51$ &   110.8 &    25.5 &    4.51 &    0.49 &   107.5 &    31.4 &    4.69 &    0.61 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4187.80 &  2.42 & $ -0.51$ &   128.5 &    28.8 &    4.82 &    0.55 &    95.9 &    27.2 &    4.42 &    0.54 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4191.43 &  2.47 & $ -0.67$ &   116.5 &    28.4 &    4.81 &    0.54 &    86.2 &    21.2 &    4.46 &    0.41 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4195.33 &  3.33 & $ -0.49$ & \nodata & \nodata & \nodata & \nodata &    60.1 &    18.7 &    4.90 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4216.18 &  0.00 & $ -3.36$ & \nodata & \nodata & \nodata & \nodata &   132.6 &    29.5 &    5.03 &    0.62 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4222.21 &  2.45 & $ -0.91$ &   107.3 &    28.8 &    4.84 &    0.55 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4233.60 &  2.48 & $ -0.58$ &   115.5 &    27.1 &    4.70 &    0.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4250.12 &  2.47 & $ -0.38$ &   119.5 &    31.8 &    4.56 &    0.59 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4282.40 &  2.18 & $ -0.78$ &   116.0 &    27.2 &    4.52 &    0.53 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4337.05 &  1.56 & $ -1.70$ &   136.9 &    33.7 &    5.00 &    0.61 &   128.3 &    40.8 &    5.18 &    0.80 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4352.73 &  2.22 & $ -1.29$ &   113.5 &    23.3 &    5.01 &    0.45 &    96.7 &    21.7 &    4.95 &    0.44 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4407.71 &  2.18 & $ -1.97$ &    78.4 &    18.9 &    5.02 &    0.30 &    79.0 &    17.9 &    5.25 &    0.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4422.57 &  2.85 & $ -1.11$ &    58.3 &    18.3 &    4.71 &    0.27 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4427.31 &  0.05 & $ -2.92$ & \nodata & \nodata & \nodata & \nodata &   135.4 &    26.2 &    4.63 &    0.53 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4430.61 &  2.22 & $ -1.66$ &    78.5 &    19.3 &    4.76 &    0.31 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4442.34 &  2.20 & $ -1.23$ &   108.9 &    24.8 &    4.80 &    0.47 &    82.2 &    19.4 &    4.59 &    0.34 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4447.72 &  2.22 & $ -1.34$ &   112.8 &    23.4 &    5.01 &    0.44 &   108.1 &    22.4 &    5.19 &    0.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4459.12 &  2.18 & $ -1.28$ &   120.4 &    24.5 &    5.04 &    0.45 &   120.7 &    26.6 &    5.33 &    0.52 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4461.65 &  0.09 & $ -3.19$ & \nodata & \nodata & \nodata & \nodata &   154.9 &    29.9 &    5.31 &    0.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4476.02 &  2.85 & $ -0.82$ &    96.3 &    18.7 &    5.00 &    0.33 &    74.4 &    19.0 &    4.84 &    0.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4484.22 &  3.60 & $ -0.86$ &    47.0 &    13.3 &    5.22 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4489.74 &  0.12 & $ -3.90$ & \nodata & \nodata & \nodata & \nodata &   108.5 &    26.1 &    5.13 &    0.52 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4494.56 &  2.20 & $ -1.14$ &   115.0 &    24.3 &    4.81 &    0.46 &   113.2 &    25.7 &    5.06 &    0.51 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4528.61 &  2.18 & $ -0.82$ & \nodata & \nodata & \nodata & \nodata &   131.1 &    29.5 &    5.06 &    0.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4531.15 &  1.48 & $ -2.10$ &   120.8 &    30.0 &    4.92 &    0.54 &   131.8 &    37.0 &    5.49 &    0.72 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4592.65 &  1.56 & $ -2.46$ &   107.5 &    19.1 &    5.15 &    0.33 &    72.4 &    17.3 &    4.86 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4602.94 &  1.49 & $ -2.21$ &   126.0 &    26.4 &    5.11 &    0.48 &    97.3 &    20.0 &    4.93 &    0.39 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4632.91 &  1.61 & $ -2.91$ &    73.5 &    14.8 &    5.13 &    0.21 &    36.4 &    10.6 &    4.83 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4647.43 &  2.95 & $ -1.35$ &    56.2 &    13.5 &    5.03 &    0.20 &    36.9 &    11.2 &    4.90 &    0.21 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4678.85 &  3.60 & $ -0.83$ &    23.4 &     7.2 &    4.75 &    0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4691.41 &  2.99 & $ -1.52$ &    43.0 &    10.3 &    5.04 &    0.17 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4707.27 &  3.24 & $ -1.08$ &    64.5 &    14.3 &    5.22 &    0.21 &    32.8 &     9.7 &    4.90 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4733.59 &  1.49 & $ -2.99$ &    72.8 &    14.3 &    5.03 &    0.20 &    54.6 &    12.8 &    5.03 &    0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4736.77 &  3.21 & $ -0.75$ &    79.3 &    15.0 &    5.06 &    0.23 &    61.2 &    13.0 &    4.98 &    0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4859.74 &  2.88 & $ -0.76$ &    83.6 &    19.5 &    4.71 &    0.30 &    85.8 &    22.0 &    4.94 &    0.38 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4871.32 &  2.87 & $ -0.36$ &   110.2 &    18.1 &    4.71 &    0.30 &   103.0 &    17.8 &    4.82 &    0.32 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4872.14 &  2.88 & $ -0.57$ &   107.1 &    18.0 &    4.88 &    0.31 &    98.7 &    17.6 &    4.96 &    0.32 &    79.1 &    17.2 &    4.73 &    0.28 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4890.76 &  2.88 & $ -0.39$ &   126.6 &    22.6 &    5.03 &    0.39 &   108.2 &    18.7 &    4.95 &    0.34 &    58.0 &    14.4 &    4.24 &    0.21 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4891.49 &  2.85 & $ -0.11$ &   110.6 &    19.3 &    4.44 &    0.33 &   105.8 &    18.2 &    4.59 &    0.33 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4903.31 &  2.88 & $ -0.93$ &    75.8 &    15.9 &    4.76 &    0.24 &    71.5 &    15.2 &    4.89 &    0.23 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4918.99 &  2.85 & $ -0.34$ &   103.5 &    20.7 &    4.55 &    0.35 &   113.4 &    22.1 &    4.95 &    0.39 &    71.7 &    16.9 &    4.35 &    0.26 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4920.50 &  2.83 & $  0.07$ &   137.4 &    25.9 &    4.69 &    0.44 &   134.7 &    26.8 &    4.90 &    0.48 &    76.7 &    17.0 &    3.99 &    0.26 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4938.81 &  2.88 & $ -1.08$ &    67.3 &    13.3 &    4.79 &    0.18 &    60.5 &    12.8 &    4.88 &    0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4939.69 &  0.86 & $ -3.25$ &   108.6 &    17.4 &    4.94 &    0.26 &    94.8 &    15.6 &    5.08 &    0.26 &    81.7 &    17.7 &    5.01 &    0.29 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4966.09 &  3.33 & $ -0.87$ &    63.4 &    16.0 &    5.09 &    0.23 &    52.3 &    13.0 &    5.09 &    0.19 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  4994.13 &  0.92 & $ -2.97$ & \nodata & \nodata & \nodata & \nodata &   125.8 &    37.8 &    5.41 &    0.69 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5006.12 &  2.83 & $ -0.61$ &    89.2 &    21.6 &    4.56 &    0.34 & \nodata & \nodata & \nodata & \nodata &    43.1 &    11.9 &    4.18 &    0.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5012.07 &  0.86 & $ -2.64$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   105.8 &    18.6 &    4.79 &    0.34 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5041.07 &  0.96 & $ -3.09$ &   140.8 &    36.2 &    5.39 &    0.56 & \nodata & \nodata & \nodata & \nodata &    63.9 &    13.4 &    4.71 &    0.19 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5041.76 &  1.49 & $ -2.20$ &   136.9 &    35.6 &    5.16 &    0.58 & \nodata & \nodata & \nodata & \nodata &   101.7 &    18.5 &    5.04 &    0.34 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5049.82 &  2.28 & $ -1.35$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    78.3 &    18.3 &    4.76 &    0.29 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5051.63 &  0.92 & $ -2.76$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   110.5 &    21.7 &    5.05 &    0.42 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5079.74 &  0.99 & $ -3.25$ &   107.2 &    27.4 &    5.07 &    0.42 & \nodata & \nodata & \nodata & \nodata &    48.8 &    13.2 &    4.68 &    0.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5083.34 &  0.96 & $ -2.84$ &   153.3 &    34.7 &    5.33 &    0.54 &   120.8 &    30.3 &    5.21 &    0.56 &    57.8 &    13.5 &    4.37 &    0.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5098.70 &  2.18 & $ -2.03$ & \nodata & \nodata & \nodata & \nodata &    57.0 &    16.0 &    4.92 &    0.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5110.41 &  0.00 & $ -3.76$ & \nodata & \nodata & \nodata & \nodata &   127.5 &    25.4 &    5.04 &    0.45 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5123.72 &  1.01 & $ -3.06$ &   129.9 &    29.3 &    5.24 &    0.46 &    94.3 &    22.5 &    5.04 &    0.38 &    57.5 &    12.8 &    4.64 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5127.36 &  0.92 & $ -3.25$ &   107.8 &    26.5 &    4.97 &    0.40 &    89.5 &    23.9 &    5.04 &    0.39 &    53.6 &    13.5 &    4.67 &    0.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5133.69 &  4.18 & $  0.14$ &    56.0 &    18.7 &    5.02 &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5142.93 &  0.96 & $ -3.08$ &   117.9 &    26.6 &    5.01 &    0.39 &   117.0 &    27.2 &    5.38 &    0.51 &    75.9 &    16.6 &    4.85 &    0.26 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5150.84 &  0.99 & $ -3.04$ &   125.3 &    28.0 &    5.11 &    0.43 &   115.0 &    24.2 &    5.34 &    0.45 &    37.9 &     9.0 &    4.31 &    0.15 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5151.91 &  1.01 & $ -3.32$ &    94.4 &    23.0 &    4.97 &    0.33 &    65.9 &    19.7 &    4.88 &    0.28 &    34.6 &     8.8 &    4.56 &    0.17 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5166.28 &  0.00 & $ -4.12$ & \nodata & \nodata & \nodata & \nodata &    97.2 &    25.0 &    4.87 &    0.42 & \nodata & \nodata & \nodata & \nodata &   106.6 &    34.1 &    6.12 &    0.68 \\
Fe I  &  5171.60 &  1.49 & $ -1.72$ &   152.0 &    33.2 &    4.88 &    0.53 &   148.5 &    37.9 &    5.26 &    0.69 &    96.5 &    19.3 &    4.45 &    0.33 &   116.0 &    43.7 &    5.58 &    0.86 \\
Fe I  &  5191.45 &  3.04 & $ -0.55$ &    87.7 &    18.9 &    4.72 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5192.34 &  3.00 & $ -0.42$ &    96.7 &    21.8 &    4.67 &    0.35 &   109.2 &    29.6 &    5.10 &    0.51 &    61.1 &    13.5 &    4.44 &    0.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5194.94 &  1.56 & $ -2.02$ &   141.3 &    29.6 &    5.11 &    0.47 &    85.5 &    21.6 &    4.54 &    0.35 &    62.5 &    14.3 &    4.33 &    0.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5198.71 &  2.22 & $ -2.09$ &    66.2 &    19.4 &    4.92 &    0.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5202.34 &  2.18 & $ -1.87$ & \nodata & \nodata & \nodata & \nodata &    89.5 &    21.8 &    5.22 &    0.37 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5216.27 &  1.61 & $ -2.08$ &   123.9 &    22.6 &    4.94 &    0.37 &   102.7 &    21.8 &    4.93 &    0.38 &    66.7 &    13.6 &    4.51 &    0.19 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5217.39 &  3.21 & $ -1.16$ &    64.9 &    14.8 &    5.22 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5232.94 &  2.94 & $ -0.06$ & \nodata & \nodata & \nodata & \nodata &   122.3 &    26.6 &    4.89 &    0.45 &    73.8 &    14.5 &    4.18 &    0.22 &   106.9 &    34.5 &    5.25 &    0.60 \\
Fe I  &  5250.21 &  0.12 & $ -4.94$ & \nodata & \nodata & \nodata & \nodata &    61.8 &    18.2 &    5.33 &    0.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5250.65 &  2.20 & $ -2.18$ &    63.0 &    17.1 &    4.94 &    0.23 &    58.5 &    17.5 &    5.10 &    0.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5254.96 &  0.11 & $ -4.76$ & \nodata & \nodata & \nodata & \nodata &    76.6 &    19.2 &    5.33 &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5266.56 &  3.00 & $ -0.39$ &   114.8 &    26.0 &    4.91 &    0.42 &    89.3 &    21.7 &    4.73 &    0.36 &    54.9 &    11.7 &    4.31 &    0.17 &    67.4 &    23.2 &    4.96 &    0.40 \\
Fe I  &  5269.54 &  0.86 & $ -1.33$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   173.5 &    25.1 &    4.65 &    0.44 &   177.6 &    47.0 &    5.39 &    0.64 \\
Fe I  &  5281.79 &  3.04 & $ -0.83$ &    60.6 &    12.7 &    4.62 &    0.17 &    60.7 &    16.3 &    4.80 &    0.24 &    42.7 &    10.0 &    4.62 &    0.17 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5283.62 &  3.24 & $ -0.52$ &    79.9 &    15.7 &    4.82 &    0.23 & \nodata & \nodata & \nodata & \nodata &    36.1 &     9.4 &    4.44 &    0.17 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5302.30 &  3.28 & $ -0.72$ &    64.1 &    15.8 &    4.85 &    0.22 &    43.8 &    11.2 &    4.73 &    0.18 & \nodata & \nodata & \nodata & \nodata &    81.1 &    29.9 &    5.82 &    0.50 \\
Fe I  &  5307.36 &  1.61 & $ -2.91$ &    75.6 &    14.7 &    5.07 &    0.19 &    82.0 &    19.3 &    5.42 &    0.30 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5324.18 &  3.21 & $ -0.10$ &   104.1 &    22.4 &    4.71 &    0.36 &   101.1 &    20.2 &    4.88 &    0.34 &    59.7 &    11.4 &    4.34 &    0.16 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5328.04 &  0.92 & $ -1.47$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   151.2 &    23.9 &    4.47 &    0.45 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5328.53 &  1.56 & $ -1.85$ &   159.6 &    30.6 &    5.18 &    0.48 &   149.3 &    27.7 &    5.45 &    0.49 &    95.7 &    17.8 &    4.63 &    0.31 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5332.90 &  1.55 & $ -2.78$ &   103.0 &    22.0 &    5.23 &    0.32 &    74.1 &    17.0 &    5.11 &    0.24 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5339.93 &  3.27 & $ -0.72$ &    72.2 &    15.3 &    4.95 &    0.21 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5367.47 &  4.42 & $  0.44$ &    45.5 &    12.7 &    4.84 &    0.21 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5369.96 &  4.37 & $  0.54$ &    63.0 &    13.9 &    4.93 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5371.49 &  0.96 & $ -1.64$ & \nodata & \nodata & \nodata & \nodata &   166.0 &    27.2 &    4.75 &    0.46 &   145.8 &    21.4 &    4.58 &    0.39 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5383.37 &  4.31 & $  0.65$ &    54.2 &    12.4 &    4.62 &    0.18 &    40.1 &    11.4 &    4.53 &    0.21 & \nodata & \nodata & \nodata & \nodata &    58.5 &    19.4 &    5.20 &    0.33 \\
Fe I  &  5393.17 &  3.24 & $ -0.91$ &    60.7 &    15.1 &    4.94 &    0.21 &    60.8 &    17.2 &    5.12 &    0.25 &    26.1 &     7.3 &    4.64 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5397.13 &  0.92 & $ -1.98$ & \nodata & \nodata & \nodata & \nodata &   164.2 &    30.4 &    5.00 &    0.52 &   136.4 &    19.1 &    4.69 &    0.35 &   125.1 &    31.2 &    5.35 &    0.61 \\
Fe I  &  5405.77 &  0.99 & $ -1.85$ & \nodata & \nodata & \nodata & \nodata &   139.4 &    24.5 &    4.53 &    0.44 &   119.0 &    17.8 &    4.32 &    0.33 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5415.20 &  4.39 & $  0.64$ &    40.9 &    11.7 &    4.53 &    0.21 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5424.07 &  4.32 & $  0.52$ &    55.0 &    13.5 &    4.78 &    0.21 &    62.1 &    14.3 &    5.00 &    0.22 &    26.3 &     6.7 &    4.48 &    0.16 &    97.0 &    27.4 &    6.00 &    0.46 \\
Fe I  &  5429.70 &  0.96 & $ -1.88$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   118.5 &    19.6 &    4.30 &    0.37 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5434.52 &  1.01 & $ -2.13$ & \nodata & \nodata & \nodata & \nodata &   171.2 &    28.3 &    5.37 &    0.48 &   102.2 &    18.9 &    4.33 &    0.32 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5446.92 &  0.99 & $ -1.91$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   123.3 &    19.2 &    4.46 &    0.35 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5455.61 &  1.01 & $ -2.09$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   124.2 &    20.7 &    4.68 &    0.37 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5497.52 &  1.01 & $ -2.83$ &   157.3 &    26.1 &    5.32 &    0.39 &   111.3 &    22.2 &    5.04 &    0.38 &    65.7 &    12.1 &    4.49 &    0.17 &    89.3 &    29.1 &    5.59 &    0.58 \\
Fe I  &  5501.47 &  0.96 & $ -3.05$ &   126.4 &    19.6 &    5.02 &    0.29 &   117.3 &    23.5 &    5.29 &    0.40 &    52.5 &    10.0 &    4.47 &    0.15 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5506.78 &  0.99 & $ -2.79$ &   138.1 &    20.1 &    4.97 &    0.29 &   120.8 &    22.1 &    5.12 &    0.39 &    74.5 &    12.9 &    4.55 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5569.62 &  3.42 & $ -0.54$ &    58.6 &    12.7 &    4.76 &    0.18 &    56.7 &    12.2 &    4.89 &    0.18 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5572.84 &  3.40 & $ -0.28$ &    86.2 &    15.4 &    4.84 &    0.21 &    72.1 &    15.1 &    4.83 &    0.22 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5576.09 &  3.43 & $ -1.00$ &    39.1 &     9.4 &    4.95 &    0.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5586.76 &  3.37 & $ -0.14$ &    84.1 &    15.2 &    4.63 &    0.22 &    71.5 &    13.8 &    4.64 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5615.64 &  3.33 & $  0.05$ &   113.7 &    18.7 &    4.82 &    0.29 &    79.0 &    16.5 &    4.51 &    0.25 &    84.9 &    16.3 &    4.67 &    0.26 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5624.54 &  3.42 & $ -0.76$ &    55.7 &    10.2 &    4.93 &    0.14 &    44.1 &    10.6 &    4.93 &    0.17 &    30.2 &     7.1 &    4.77 &    0.14 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5658.82 &  3.40 & $ -0.79$ &    45.2 &    11.0 &    4.79 &    0.17 &    29.9 &     8.4 &    4.69 &    0.17 &    25.8 &     6.2 &    4.69 &    0.15 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  5701.54 &  2.56 & $ -2.14$ &    33.9 &     8.5 &    4.90 &    0.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6065.48 &  2.61 & $ -1.41$ &    86.3 &    13.6 &    4.92 &    0.18 &    64.9 &    11.4 &    4.86 &    0.16 &    43.0 &     9.1 &    4.65 &    0.15 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6136.61 &  2.45 & $ -1.41$ &   104.0 &    15.0 &    4.94 &    0.21 &    98.7 &    15.6 &    5.14 &    0.25 &    56.5 &     9.5 &    4.65 &    0.14 &    87.7 &    21.1 &    5.71 &    0.39 \\
Fe I  &  6137.69 &  2.59 & $ -1.35$ &   100.1 &    14.9 &    5.01 &    0.20 &    80.6 &    13.4 &    4.99 &    0.20 &    35.5 &     6.7 &    4.44 &    0.12 &    71.6 &    19.7 &    5.51 &    0.36 \\
Fe I  &  6191.56 &  2.43 & $ -1.42$ &   113.4 &    16.4 &    5.05 &    0.24 &    85.1 &    13.8 &    4.92 &    0.21 &    58.0 &    10.1 &    4.65 &    0.14 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6200.31 &  2.61 & $ -2.44$ & \nodata & \nodata & \nodata & \nodata &    22.6 &     6.0 &    5.20 &    0.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6213.43 &  2.22 & $ -2.48$ &    60.5 &    10.2 &    5.15 &    0.13 &    34.2 &     7.4 &    4.99 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6219.28 &  2.20 & $ -2.45$ &    58.8 &    10.1 &    5.07 &    0.13 &    52.7 &     9.1 &    5.22 &    0.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6230.72 &  2.56 & $ -1.28$ &    94.1 &    13.7 &    4.81 &    0.19 &    81.6 &    13.3 &    4.89 &    0.20 &    43.8 &     9.0 &    4.46 &    0.14 &    72.0 &    25.5 &    5.41 &    0.46 \\
Fe I  &  6246.32 &  3.60 & $ -0.88$ &    46.4 &     9.6 &    5.11 &    0.15 &    35.1 &     6.9 &    5.09 &    0.12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6252.56 &  2.40 & $ -1.69$ &   103.3 &    15.8 &    5.13 &    0.22 &    82.5 &    12.5 &    5.11 &    0.18 &    36.4 &     7.1 &    4.56 &    0.13 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6254.26 &  2.28 & $ -2.44$ &    56.6 &    10.4 &    5.14 &    0.14 &    45.7 &     9.2 &    5.21 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6265.13 &  2.18 & $ -2.54$ &    62.5 &     9.6 &    5.18 &    0.12 &    42.0 &     8.6 &    5.13 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6301.50 &  3.65 & $ -0.72$ &    47.9 &    10.2 &    5.03 &    0.16 &    47.5 &    12.9 &    5.18 &    0.21 &    26.9 &     5.6 &    4.91 &    0.12 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6335.33 &  2.20 & $ -2.18$ &    64.6 &    11.1 &    4.87 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6336.84 &  3.69 & $ -1.05$ & \nodata & \nodata & \nodata & \nodata &    21.4 &     5.6 &    5.08 &    0.15 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6393.60 &  2.43 & $ -1.58$ &    97.7 &    13.2 &    4.97 &    0.19 &    79.9 &    12.4 &    4.99 &    0.18 &    35.5 &     7.2 &    4.46 &    0.13 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6400.00 &  3.60 & $ -0.29$ & \nodata & \nodata & \nodata & \nodata &    70.7 &    11.7 &    5.01 &    0.17 &    34.9 &    10.5 &    4.56 &    0.20 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6411.65 &  3.65 & $ -0.59$ & \nodata & \nodata & \nodata & \nodata &    47.4 &     9.2 &    5.04 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6421.35 &  2.28 & $ -2.01$ &    86.0 &    12.2 &    5.06 &    0.15 &    72.9 &    12.1 &    5.14 &    0.17 &    19.2 &     4.1 &    4.38 &    0.12 &    52.0 &    13.9 &    5.48 &    0.24 \\
Fe I  &  6430.85 &  2.18 & $ -1.95$ &    71.1 &    10.5 &    4.68 &    0.13 &    92.7 &    13.6 &    5.23 &    0.20 &    46.8 &     7.5 &    4.70 &    0.11 &    52.1 &    13.9 &    5.31 &    0.24 \\
Fe I  &  6494.98 &  2.40 & $ -1.24$ &   121.2 &    18.2 &    4.90 &    0.25 &   112.8 &    17.1 &    5.10 &    0.27 &    59.8 &     9.1 &    4.44 &    0.13 &    96.8 &    18.9 &    5.63 &    0.35 \\
Fe I  &  6498.94 &  0.96 & $ -4.70$ & \nodata & \nodata & \nodata & \nodata &    25.8 &     6.9 &    5.48 &    0.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6592.91 &  2.73 & $ -1.47$ &    71.2 &    11.1 &    4.90 &    0.14 &    56.1 &     9.4 &    4.92 &    0.13 &    33.4 &     8.4 &    4.67 &    0.16 &    75.1 &    21.2 &    5.83 &    0.39 \\
Fe I  &  6593.87 &  2.44 & $ -2.37$ &    46.3 &     8.8 &    5.11 &    0.13 &    24.6 &     6.0 &    4.95 &    0.15 &    16.7 &     5.0 &    4.85 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6663.44 &  2.42 & $ -2.48$ &    35.0 &     6.6 &    5.02 &    0.12 &    34.8 &     7.6 &    5.22 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6677.99 &  2.69 & $ -1.42$ &    91.3 &    12.8 &    5.04 &    0.17 &    70.7 &    11.5 &    5.01 &    0.16 &    28.6 &     5.7 &    4.48 &    0.12 &    62.3 &    15.0 &    5.51 &    0.26 \\
Fe I  &  6750.15 &  2.42 & $ -2.58$ &    31.1 &     7.2 &    5.05 &    0.14 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe I  &  6978.85 &  2.48 & $ -2.45$ &    29.1 &     6.0 &    4.94 &    0.12 &    25.9 &     6.8 &    5.08 &    0.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4233.17 &  2.58 & $ -1.97$ &   115.3 &    28.5 &    4.99 &    0.58 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4508.28 &  2.86 & $ -2.58$ &    69.8 &    14.2 &    5.09 &    0.22 &    74.2 &    16.5 &    5.40 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4515.34 &  2.84 & $ -2.60$ &    77.6 &    17.3 &    5.20 &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4520.22 &  2.81 & $ -2.60$ &    75.0 &    17.8 &    5.12 &    0.29 &    60.0 &    17.9 &    5.14 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4522.63 &  2.84 & $ -2.25$ &    71.3 &    17.5 &    4.75 &    0.28 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4555.89 &  2.83 & $ -2.40$ & \nodata & \nodata & \nodata & \nodata &    71.8 &    17.7 &    5.14 &    0.29 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4583.84 &  2.81 & $ -1.93$ &    82.7 &    16.9 &    4.57 &    0.28 &    71.9 &    15.6 &    4.65 &    0.26 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Fe II &  4923.93 &  2.89 & $ -1.32$ &   122.9 &    27.4 &    4.68 &    0.51 &   121.5 &    24.1 &    4.96 &    0.46 &    94.2 &    18.8 &    4.34 &    0.33 & \nodata & \nodata & \nodata & \nodata \\
Fe II &  5018.45 &  2.89 & $ -1.22$ &   127.2 &    32.2 &    4.65 &    0.59 &   115.4 &    33.2 &    4.72 &    0.63 &    84.7 &    17.7 &    4.08 &    0.29 & \nodata & \nodata & \nodata & \nodata \\
Fe II &  5169.03 &  2.89 & $ -1.00$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &   164.0 &    50.2 &    5.98 &    0.82 \\
Fe II &  5197.58 &  3.23 & $ -2.22$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    36.9 &     9.7 &    4.76 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Fe II &  5234.63 &  3.22 & $ -2.18$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &    43.4 &    11.0 &    4.81 &    0.18 & \nodata & \nodata & \nodata & \nodata \\
Fe II &  5276.00 &  3.20 & $ -2.01$ &    96.9 &    18.5 &    5.27 &    0.29 &    63.6 &    15.1 &    5.03 &    0.23 &    53.9 &    10.9 &    4.77 &    0.16 & \nodata & \nodata & \nodata & \nodata \\
Fe II &  6456.38 &  3.90 & $ -2.08$ &    23.9 &     6.3 &    5.00 &    0.16 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  3995.31 &  0.92 & $ -0.22$ &   135.7 &    39.3 &    2.66 &    0.76 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  4118.77 &  1.05 & $ -0.49$ &   126.6 &    38.1 &    2.87 &    0.71 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Co I  &  4121.32 &  0.92 & $ -0.32$ &   138.8 &    33.8 &    2.75 &    0.63 &   123.4 &    35.6 &    2.86 &    0.74 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  4714.42 &  3.38 & $  0.23$ &    52.0 &    11.9 &    3.63 &    0.18 &    52.6 &    13.0 &    3.79 &    0.20 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  5137.07 &  1.68 & $ -1.99$ &    67.1 &    18.0 &    3.88 &    0.24 & \nodata & \nodata & \nodata & \nodata &    40.0 &     9.0 &    3.83 &    0.15 & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  5476.90 &  1.83 & $ -0.89$ &   151.8 &    23.7 &    4.19 &    0.38 &   115.2 &    23.1 &    3.93 &    0.43 &    84.9 &    18.3 &    3.53 &    0.30 & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  5754.68 &  1.94 & $ -2.33$ &    30.4 &     7.5 &    3.97 &    0.15 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  6108.12 &  1.68 & $ -2.45$ &    35.2 &     7.6 &    3.82 &    0.14 &    28.7 &     6.4 &    3.93 &    0.13 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ni I  &  6643.64 &  1.68 & $ -2.30$ &    65.4 &    10.4 &    4.04 &    0.13 &    45.5 &     7.9 &    4.02 &    0.12 &    29.9 &     5.4 &    3.88 &    0.11 &     syn & \nodata &$  <5.36$& \nodata \\
Ni I  &  6767.77 &  1.83 & $ -2.17$ &    52.2 &     7.9 &    3.92 &    0.11 &    43.4 &     8.0 &    4.04 &    0.12 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Zn I  &  4810.53 &  4.08 & $ -0.14$ &    22.7 &     6.8 &    1.95 &    0.18 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sr II &  4077.71 &  0.00 & $  0.15$ &     syn & \nodata &   -1.85 &    0.50 &     syn & \nodata &   -1.75 &    0.50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Sr II &  4215.52 &  0.00 & $ -0.18$ &     syn & \nodata &   -1.45 &    0.50 &     syn & \nodata &   -1.55 &    0.50 & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Ba II &  4554.03 &  0.00 & $  0.16$ &     syn & \nodata &   -2.22 &    0.20 &     syn & \nodata &   -1.05 &    0.30 &     syn & \nodata &$ <-1.29$& \nodata & \nodata & \nodata & \nodata & \nodata \\
Ba II &  4934.09 &  0.00 & $ -0.16$ &     syn & \nodata &   -2.45 &    0.20 &     syn & \nodata &   -1.40 &    0.25 &     syn & \nodata &$ <-2.22$& \nodata & \nodata & \nodata & \nodata & \nodata \\
Ba II &  6141.71 &  0.70 & $ -0.08$ &     syn & \nodata &   -1.76 &    0.10 &     syn & \nodata &   -1.22 &    0.20 &     syn & \nodata &$ <-1.89$& \nodata &     syn & \nodata &$ <-0.06$& \nodata \\
Ba II &  6496.90 &  0.60 & $ -0.37$ &     syn & \nodata &   -1.81 &    0.15 &     syn & \nodata &   -1.21 &    0.15 &     syn & \nodata &$ <-1.75$& \nodata &     syn & \nodata &$ <-0.02$& \nodata \\
Eu II &  4129.72 &  0.00 & $  0.22$ &     syn & \nodata &$ <-1.68$& \nodata &     syn & \nodata &$ <-1.20$& \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata \\
Eu II &  6645.06 &  1.38 & $  0.12$ & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata & \nodata &     syn & \nodata &$ <-0.89$& \nodata &     syn & \nodata &$  <0.50$& \nodata \\
\enddata
\end{deluxetable*}

